VLG: General Video Recognition with Web Textual Knowledge

Video recognition in an open and dynamic world is quite challenging, as we need to handle different settings such as close-set, long-tail, few-shot and open-set. By leveraging semantic knowledge from noisy text descriptions crawled from the Internet, we focus on the general video recognition (GVR) problem of solving different recognition tasks within a unified framework. The core contribution of this paper is twofold. First, we build a comprehensive video recognition benchmark of Kinetics-GVR, including four sub-task datasets to cover the mentioned settings. To facilitate the research of GVR, we propose to utilize external textual knowledge from the Internet and provide multi-source text descriptions for all action classes. Second, inspired by the flexibility of language representation, we present a unified visual-linguistic framework (VLG) to solve the problem of GVR by an effective two-stage training paradigm. Our VLG is first pre-trained on video and language datasets to learn a shared feature space, and then devises a flexible bi-modal attention head to collaborate high-level semantic concepts under different settings. Extensive results show that our VLG obtains the state-of-the-art performance under four settings. The superior performance demonstrates the effectiveness and generalization ability of our proposed framework. We hope our work makes a step towards the general video recognition and could serve as a baseline for future research. The code and models will be available at https://github.com/MCG-NJU/VLG.

==> tables/different_m.tex <==
\begin{tabular}{c|c|c|c|c|c|c}
    \shline
    Dataset & Backbone & $M$ & Top-1 & Many & Medium & Few \\
    \multirow{4}{*}{Kinetics-LT} & \multirow{4}{*}{ResNet-50} & 16 & 58.1 & 73.1 & 58.4 & 39.2 \\
    \multirow{4}{*}{Kinetics-LT} & \multirow{4}{*}{ResNet-50} & 32 & 58.1 & 73.2 & 58.5 & 39.2 \\
    \multirow{4}{*}{Kinetics-LT} & \multirow{4}{*}{ResNet-50} & 64 & 58.7 & 73.2 & 58.7 & 38.8 \\
    \multirow{4}{*}{Kinetics-LT} & \multirow{4}{*}{ResNet-50} & 128 & 57.9 & 73.2 & 58.7 & 38.8 \\
    \multirow{4}{*}{Kinetics-LT} & \multirow{4}{*}{ResNet-50} & 256 & 57.8 & 73.2 & 58.7 & 38.8 \\
\end{tabular}

==> tables/hmdb51_results.tex <==
\begin{tabular}{c|c|c|c|c|c|c}
    \shline
    Method & Pretrain & Backbone & Frame & Views & Top-1 & Top-5 \\
    \shline
    \multirow{3}{*}{VLG} & \multirow{3}{*}{$\text{CLIP}^*$+K400} & \multirow{3}{*}{ViT-B/16} & 8 & $1 \times 1$ & 71.7 & 92.2 \\
     & & & 16 & $1 \times 1$ & 71.7 & 91.9 \\
     & & & 16 & $4 \times 3$ & \textbf{71.7} & \textbf{92.8} \\
    \shline
    \multirow{3}{*}{VLG} & \multirow{3}{*}{$\text{CLIP}^*$+K400} & \multirow{3}{*}{ViT-L/14} & 8 & $1 \times 1$ & 73.1 & 92.7 \\
    & & & 16 & $1 \times 1$ & \textbf{73.2} & 93.0 \\
    & & & 16 & $4 \times 3$ & 72.4 & \textbf{93.2} \\
    \shline
\end{tabular}
